The Path to Fault- and Intrusion-Resilient Manycore Systems on a Chip

The hardware computing landscape is changing. What used to be distributed systems can now be found on a chip with highly configurable, diverse, specialized and general purpose units. Such Systems-on-a-Chip (SoC) are used to control today's cyber-physical systems, being the building blocks of critical infrastructures. They are deployed in harsh environments and are connected to the cyberspace, which makes them exposed to both accidental faults and targeted cyberattacks. This is in addition to the changing fault landscape that continued technology scaling, emerging devices and novel application scenarios will bring. In this paper, we discuss how the very features, distributed, parallelized, reconfigurable, heterogeneous, that cause many of the imminent and emerging security and resilience challenges, also open avenues for their cure though SoC replication, diversity, rejuvenation, adaptation, and hybridization. We show how to leverage these techniques at different levels across the entire SoC hardware/software stack, calling for more research on the topic.

==> intro.tex <==
\section{A New Computing Landscape}
\label{sec:intro}

\stb{1pg}{
  \begin{itemize}
  \item come up with better title
  \item changing hardware landscape
    \begin{itemize}
    \item computing benefits from processing inaccurately (not always clear how this affects failures)
    \item performance through speculation => timing inaccuracy
    \item emerging devices (Silicon nanowire, carbon nanotube, ...) will initially show less reliability
    \end{itemize}
  \item heterogeneity
    \begin{itemize}
    \item big little
    \item accelerators for ...
    \item stacking / chiplets / ... => side effects on nearby computation (heat, ...)
    \end{itemize}
  \item role of proximity faults in modern systems
  \item novel application areas: new space, ...
  \end{itemize}}

	What used to be distributed systems, filling data centers two to three decades ago can now readily be found on many-core systems on a chip (MPSoCs). MPSoCs are charged to control critical infrastructure, cyber-physical systems or to manage high-value digital assets, financial and others, including what probably constitutes our most sensitive and valuable information: our genome.
	%
 	They integrate general purpose cores and special processing elements (such as signal processors, GPGPU cores, and tensor units) and they consolidate these units on a single chip, a 3D stack of the same or as a more loose coupling, by leveraging chiplet optical and other interconnects~\cite{ucie}.

 	Today's extraordinary performance is achieved through parallelization and speculation, with all problems that this entails (side channels, timing anomalies, "waste" of power when discarding roughly half of the computed values, etc.). 
 	Some of the emerging technologies (whether 1D transistors, such as silicon nanowires, carbon nanotubes or graphene, or beyond Moore computing paradigms, such as spintronic racetrack) bear the potential to revolutionize this performance landscape, albeit at the cost of largely differing failure characteristics, which renews the recurring question to what extend hardware should mitigate faults or where software might take over.
 	%
 	Organic computing~\cite{10.1007/978-3-642-16576-4_5} has so far favored the hardware approach to self-healing, but coarse of fine-grain reconfiguration also brought software into the game. 
 	
 	So what is at stake? 
  %
  We might of course choose to continue considering hardware development a separate discipline with marginal overlap to dependability, allowing chips to be manufactured with performance and energy consumption as primary optimization targets, and use them in the worst case as one indivisible fault containment domain with all its implications. 
  %
  For example, autonomous vehicles would come with $2f+1$ physically separated "brains", voting on independently generated trajectories, when each individually would already bring the resources for resilient autonomous driving. 
  %
  Or, we might engage and accept the challenges ahead of us to take future multi- and many-core systems on a chip as what they are: distributed systems on a chip with all their fault containment, fault tolerance and resilience potential that we learned to understand from their large scale counterparts. 

  In this position paper and call to action, we take the latter route and ask what is necessary to turn MPSoCs into a foundation for resilient computing. We discuss challenges and early solutions, programmability, elasticity and plasticity, the role of adaptation and how to obtain it.


==> models.tex <==
\section{System and Fault Model}

\stb{1 paragraph}{Overview}

\stb{1 paragraph}{
  Goals and Non-Goals: 
  \begin{itemize}
  \item Hardware / software co-design for resilience
  \item In perspective of new material circuits, re-evaluate current
    HW software contracts (where to catch faults)
  \item consider both fixed function and reconfigurable logic 
  \item anticipate emerging circuit technologies (SiNW, CNT, Racetrack, Quantum, ...)
  \item we disregard a large class of proximity faults, such as physical
    impact, etc., but not PE-to-PE effects.
  \end{itemize}
}

\stb{1 paragraph}{
  System Model and Assumptions:
  \begin{itemize}
  \item system comprised of fixed function + dynamic processing elements
  \item PEs connected by on-chip, cross chiplet, chip-to-chip
    interconnects (optical, TSVs, ...) and possibly 3D stacked
  \item adversaries may target hardware, software, combination of the
    two (in particular as hardware/software line blurs due to
    reconfiguration, microcode, ...)
  \item assume hardware can and will fail like software, possibly with
    different statistics as far as accidental faults are occured =>
    the more complex the more likely to fail
  \end{itemize}
}

In this paper, we consider systems comprised of fixed-function or dynamically-programmed processing elements (PEs), realized on chip, on chiplets or as a multiprocessing systems comprised of multiple physically co-located and possibly stacked chips. 
PEs are interconnected (e.g., through on-chip or chip-to-chip interconnects, through silicon vias or optical waveguides) and may run an arbitrary combination of specific or general purpose applications, depending on the type of PE. In particular, we anticipate that at some stage PEs with emerging circuit technologies will be integrated, possibly together with traditional CMOS circuits, but built from Silicon Nanowires, Carbon Nanotubes, sheets of Graphene, etc. with their unique fault characteristics. We may also see technologies such as Racetrack spintronic storage or quantum elements or even processing elements that bridge into the biological or chemical domain. 

We consider adversaries to target all levels of the hardware/software stack, in particular as configurable logic blurs the line between the two. Accidental faults are likely to show significantly different characteristics and may require specific solutions (e.g., to avoid decoherence effects in the quantum realm). Obviously, tightly co-located systems cannot tolerate proximity faults with effect radi larger than the system's fault containment domains (e.g., physical impact or power supply errors (if a single central source is used) versus particle impacts to individual transistors or PEs). 

We shall see that some single-points-of-failure (SPOFs) are inevitable for some of the designs we envision. For those, we will follow, without having fully established evidence, the line of argumentation we typically use to justify hybrid fault models. Namely, the simpler a circuit, the less likely it is to fail, which we believe will hold in general down to a minimal complexity for most circuits at hand, but obviously not for all. For example, bit flips in a simple register are likely fatal and will require the minimal complexity of register-level ECC (i.e., extra bits and logic), but our argument is likely to hold once circuits are protected in that manner. A dual argument applies when looking at the problem from the other end of the spectrum. At some stage fixed-function hardware exceeds in complexity what is required to fetch, decode and execute instructions. Once trusted components exceed this complexity, software solutions, running on simple processors, become the element of choice for realizing trustworthy functionality, so again, like with the trusted components of the BFT-SMR protocols the dependability community used to develop~\cite{6081855,7307998,1353018,10.1145/3492321.3519568} the question becomes what functionality is required and will it remain sufficiently simple to allow implementing it in fixed-function hardware. 

%\section{Hardware-Level Attacks}



